Mirage Models Confront the LHC: I. Kahler-Stabilized Heterotic String Theory

We begin the study of a class of string-motivated effective supergravity theories in light of current data from the CERN Large Hadron Collider (LHC). The case of heterotic string theory, in which the dilaton is stabilized via non-perturbative corrections to the Kahler metric, will be considered first. This model is highly constrained and therefore predictive. We find that much of the reasonable parameter space afforded to the model -- representing the strong dynamics of a presumed gaugino condensation in the hidden sector -- is now observationally disfavored by the LHC results. Most of the theoretically-motivated parameter space that remains can be probed with data that has already been collected, and most of the remainder will be definitively explored within the first year of operation at center of mass energy of 13 TeV. Expected signatures for a number of benchmark points are discussed. We find that the surviving space of the model makes a precise prediction as to the relation of many superpartner masses, as well as the manner in which the correct dark matter relic density is obtained. Implications for current and future dark matter search experiments are discussed.

==> Final Draft/basic.tex <==
%%%%%%%%%%%%%%%%%%%%%%%
% Command definitions %
%%%%%%%%%%%%%%%%%%%%%%%

% This defines a small-caps format for use in math mode (equations)
\DeclareMathAlphabet   {\mathsc}{OT1}{cmr}{m}{sc}

% Define new formatting functions
\newcommand{\nochapter}[1]{
  \chapter*{#1}
  \markboth{#1}{#1}
  \addcontentsline{toc}{chapter}{#1}}
\newcommand{\nnn}{ \nonumber \\ }
%\newcommand{\eqref}[1]{~(\ref{#1})}
\newcommand{\sgspace}{\def\baselinestretch{1.0}}
\newcommand{\dbspace}{\def\baselinestretch{1.8}}
% Left and right formatting
\def\[{\left [}
\def\]{\right ]}
\def\({\left (}
\def\){\right )}
\newcommand{\lang}{\left\langle}
\newcommand{\rang}{\right\rangle}
\newcommand{\lbr}{\left\{}
\newcommand{\rbr}{\right\}}
% Barred quantities
\newcommand{\oline}[1]{\overline{#1}}
\newcommand{\jbar}{\bar{\jmath}}
\newcommand{\ibar}{\bar{\imath}}
% Tildes
\newcommand{\td}[1]{\tilde{#1}}
\newcommand{\wtd}[1]{\widetilde{#1}}
% Caligraphy
\newcommand{\Lag}{\mathcal{L}}
\newcommand{\D}{\mathcal{D}}
% Hatted quantities
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\h}[1]{\hat{#1}}
% Slashed quantities
\newcommand{\notd}{\not{\hspace{-.05in}\pp}}
\newcommand{\notD}{\not{\hspace{-.05in}D}}
\newcommand{\notcD}{\not{\hspace{-.05in}\D}}
% Useful HEP definitions
%\newcommand{\pCL}      {\%~\mathrm{C.L.}}
\newcommand{\MeV}      {~\mathrm{MeV}}
\newcommand{\GeV}      {~\mathrm{GeV}}
\newcommand{\TeV}      {~\mathrm{TeV}}
\newcommand{\MS}       {\mathsc{\overline{MS}}}
\newcommand{\SM}       {\mathsc{sm}}
\newcommand{\EW}       {\mathsc{ew}}
\newcommand{\IR}       {\mathsc{ir}}
\newcommand{\EM}       {\mathsc{em}}
\newcommand{\CP}       {\mathsc{cp}}
\newcommand{\KE}       {\mathsc{ke}}
\newcommand{\VY}       {\mathsc{vy}}
\newcommand{\UV}       {\mathsc{uv}}
\newcommand{\GS}       {\mathsc{gs}}
\newcommand{\PL}       {\mathsc{pl}}
\newcommand{\PV}       {\mathsc{pv}}
\newcommand{\GUT}      {\mathsc{gut}}
\newcommand{\STR}      {\mathsc{str}}
\newcommand{\SUSY}     {\mathsc{susy}}
\newcommand{\MSSM}     {\mathsc{mssm}}
\newcommand{\COND}     {\mathsc{cond}}
\newcommand{\Mpl}{M_{\PL}}
% Supergravity quantities
\newcommand{\superint}{\int\diff^{4}\theta}
\newcommand{\chiral}{\(\bar{\D}^2 - 8R\)}
\newcommand{\achiral}{\({\D}^2 - 8\oline{R}\)}
\newcommand{\Mgrav}{M_{3/2}}
\newcommand{\rpart}[1]{{#1}+\oline{#1}}
\newcommand{\ww}{W^\alpha W_\alpha}
\newcommand{\bww}{\overline{W}_{\dot\alpha} \overline{W}^{\dot\alpha}}
\newcommand{\WaWa}{ W_a^{\alpha} W_{b}^{\alpha}}
\newcommand{\WbWb}{ W^a_{\dot{\alpha}}W^{b\dot{\alpha}}}
\newcommand{\DaDa}{{\D}^{\alpha}{\D}_{\alpha}}
\newcommand{\DbDb}{{\D}_{\dot{\alpha}}{\D}^{\dot{\alpha}}}
\newcommand{\Da}{{\D}_{\alpha}}
\newcommand{\Db}{{\D}^{\dot{\beta}}}
\newcommand{\Dc}{{\D}^{\alpha}}
\newcommand{\Dd}{{\D}_{\dot{\beta}}}
\newcommand{\Wa}{W_{\alpha}}
\newcommand{\Wb}{W^{\dot{\beta}}}
\newcommand{\Wc}{W^{\alpha}}
\newcommand{\Wd}{W_{\dot{\beta}}}
\newcommand{\lowest}{|_{\theta =\bar{\theta}=0}}
\newcommand{\blowest}{\bigg|_{\theta =\bar{\theta}=0}}
% This last one is lowest component without any thetas
\def\Eisen{G_{2}\(t,\bar{t}\)}
\def\bli{\bigg|}
% Put alpha superscript/subscripts
\newcommand{\supal}[1]{{#1}^{\alpha}}
\newcommand{\subal}[1]{{#1}_{\alpha}}
\newcommand{\supdal}[1]{{#1}^{\dot{\alpha}}}
\newcommand{\subdal}[1]{{#1}_{\dot{\alpha}}}
% BGW model quantities
\newcommand{\baal}{b_{a}^{\alpha}}
\newcommand{\baaleff}{\(\baal\)_{\rm eff}}
\newcommand{\bpaleff}{\(b_{+}^{\alpha}\)_{\rm eff}}
\newcommand{\caleff}{\({c_{\alpha}}\)_{\rm eff}}
% Useful shortcuts in formulae
\newcommand{\lhs}      {\mbox{l.h.s.}}
\newcommand{\rhs}      {\mbox{r.h.s.}}
\newcommand{\hc}       {\mathrm{\; h.c. \;}}
\newcommand{\cc}       {\mathrm{\; c.c. \;}}
\newcommand{\pp}{\partial}
\newcommand{\Br}{{\rm Br}}
\newcommand{\Det}{{\rm Det}}
\newcommand{\STr}{{\rm STr}}
\newcommand{\Tr}{{\rm Tr}}
\newcommand{\btr}{{\bf Tr}}
\newcommand{\diff}{\mbox{d}}
\newcommand{\order}{\mathcal{O}}
\newcommand{\re}{{\rm Re}}
\newcommand{\im}{{\rm Im}}
\newcommand{\lsimeq}{{\stackrel{<}{\sim}}}
\newcommand{\gsimeq}{{\stackrel{>}{\sim}}}
%\newcommand{\loop}{{1\over16\pi^2}}
\newcommand{\loopp}{{1\over32\pi^2}}
\newcommand{\gappeq}{\mathrel{\rlap {\raise.5ex\hbox{$>$}}
{\lower.5ex\hbox{$\sim$}}}}
\newcommand{\lappeq}{\mathrel{\rlap{\raise.5ex\hbox{$<$}}
{\lower.5ex\hbox{$\sim$}}}}
\newcommand{\up}{^{(0)}}
\newcommand{\upp}{^{(1)}}

% Hyphenation list
\hyphenation{su-per-sym-me-try su-per-sym-met-ric sca-lar sca-lars
  coun-ter-term fer-mi-on fer-mi-ons gau-gi-no gau-gi-nos chi-ral
  su-per-mul-ti-plet su-per-po-ten-tial a-no-ma-ly su-per-gra-vi-ty
  non-u-ni-ver-sal non-u-ni-ver-sal-i-ties non-van-ish-ing tri-lin-ear
  bi-lin-ear La-gran-gi-ans coun-ter-terms mul-ti-plet mul-ti-plets
  spur-i-on spur-i-ons non-per-tur-ba-tive grav-i-ti-no per-turb-a-tive
  bi-fun-da-ment-al}


==> Final Draft/references.tex <==
%%%% INTRO %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{:2012gu} 
  S.~Chatrchyan {\it et al.}  [CMS Collaboration],
  %``Observation of a new boson at a mass of 125 GeV with the CMS experiment at the LHC,''
  Phys.\ Lett.\ B {\bf 716}, 30 (2012)
  [arXiv:1207.7235 [hep-ex]]; \newline
  %%CITATION = ARXIV:1207.7235;%%
%\bibitem{CMS} 
  S.~Chatrchyan {\it et al.}  [CMS Collaboration],
  %``Observation of a new boson at a mass of 125 GeV with the CMS experiment at the LHC,''
  Phys.\ Rev.\ Lett. {\bf 110}, 081803 (2013)
  [arXiv:1207.7235 [hep-ex]].
  %%CITATION = ARXIV:1207.7235;%%  
\bibitem{:2012gk} 
  G.~Aad {\it et al.}  [ATLAS Collaboration],
  %``Observation of a new particle in the search for the Standard Model Higgs boson with the ATLAS detector at the LHC,''
  Phys.\ Lett.\ B {\bf 716}, 1 (2012)
  [arXiv:1207.7214 [hep-ex]]; \newline
  %%CITATION = ARXIV:1207.7214;%%
  ATLAS-CONF-2013-024


\bibitem{:2012ct} 
  RAaij {\it et al.}  [LHCb Collaboration],
  %``First evidence for the decay Bs -> mu+ mu-,''
  arXiv:1211.2674 [Unknown].
  %%CITATION = ARXIV:1211.2674;%%

\bibitem{Choi:2007ka}
  K.~Choi and H.~P.~Nilles,
%  ``The gaugino code,''
  JHEP {\bf 0704}, 006 (2007)
  [arXiv:hep-ph/0702146].
  %%CITATION = JHEPA,0704,006;%%
\bibitem{Altunkaynak:2009tg} 
  B.~Altunkaynak, P.~Grajek, M.~Holmes, G.~Kane and B.~D.~Nelson,
  %``Studying Gaugino Mass Unification at the LHC,''
  JHEP {\bf 0904}, 114 (2009)
  [arXiv:0901.1145 [hep-ph]].
  %%CITATION = ARXIV:0901.1145;%%

\bibitem{Baer:2007uz} 
  H.~Baer, A.~Box, E.~-K.~Park and X.~Tata,
  %``Implications of compressed supersymmetry for collider and dark matter searches,''
  JHEP {\bf 0708}, 060 (2007)
  [arXiv:0707.0618 [hep-ph]].
  %%CITATION = ARXIV:0707.0618;%%
%\bibitem{LeCompte:2011cn} 
%  T.~J.~LeCompte and S.~P.~Martin,
  %``Large Hadron Collider reach for supersymmetric models with compressed mass spectra,''
%  Phys.\ Rev.\ D {\bf 84}, 015004 (2011)
%  [arXiv:1105.4304 [hep-ph]].
  %%CITATION = ARXIV:1105.4304;%%
%\bibitem{LeCompte:2011fh} 
%  T.~J.~LeCompte and S.~P.~Martin,
  %``Compressed supersymmetry after 1/fb at the Large Hadron Collider,''
%  Phys.\ Rev.\ D {\bf 85}, 035023 (2012)
%  [arXiv:1111.6897 [hep-ph]].
  %%CITATION = ARXIV:1111.6897;%%
%\bibitem{Murayama:2012jh} 
%  H.~Murayama, Y.~Nomura, S.~Shirai and K.~Tobioka,
  %``Compact Supersymmetry,''
%  arXiv:1206.4993 [hep-ph].
  %%CITATION = ARXIV:1206.4993;%%
\bibitem{Dreiner:2012gx} 
  H.~K.~Dreiner, M.~Kramer and J.~Tattersall,
  %``How low can SUSY go? Matching, monojets and compressed spectra,''
  Europhys.\ Lett.\  {\bf 99}, 61001 (2012)
  [arXiv:1207.1613 [hep-ph]].
  %%CITATION = ARXIV:1207.1613;%%  
  
\bibitem{Chamseddine:1982jx} 
  A.~H.~Chamseddine, R.~L.~Arnowitt and P.~Nath,
  %``Locally Supersymmetric Grand Unification,''
  Phys.\ Rev.\ Lett.\  {\bf 49}, 970 (1982).
  %%CITATION = PRLTA,49,970;%%
\bibitem{Nath:1983aw} 
  P.~Nath, R.~L.~Arnowitt and A.~H.~Chamseddine,
  %``Gauge Hierarchy in Supergravity Guts,''
  Nucl.\ Phys.\ B {\bf 227}, 121 (1983).
  %%CITATION = NUPHA,B227,121;%%
\bibitem{Hall:1983iz} 
  L.~J.~Hall, J.~D.~Lykken and S.~Weinberg,
  %``Supergravity as the Messenger of Supersymmetry Breaking,''
  Phys.\ Rev.\ D {\bf 27}, 2359 (1983).
  %%CITATION = PHRVA,D27,2359;%%          

\bibitem{Gaillard:2007jr}
  M.~K.~Gaillard and B.~D.~Nelson,
%  ``K\"ahler stabilized, modular invariant heterotic string models,''
  Int.\ J.\ Mod.\ Phys.\  A {\bf 22}, 1451 (2007)
  [arXiv:hep-th/0703227].
  %%CITATION = IMPAE,A22,1451;%%
\bibitem{Casas:1996zi}
  J.~A.~Casas,
%  ``The generalized dilaton supersymmetry breaking scenario,''
  Phys.\ Lett.\  B {\bf 384}, 103 (1996)
  [arXiv:hep-th/9605180].
  %%CITATION = PHLTA,B384,103;%%
\bibitem{Binetruy:1996xja}
  P.~Binetruy, M.~K.~Gaillard and Y.~Y.~Wu,
%  ``Dilaton Stabilization in the Context of Dynamical Supersymmetry Breaking
%  through Gaugino Condensation,''
  Nucl.\ Phys.\  B {\bf 481}, 109 (1996)
  [arXiv:hep-th/9605170].
  %%CITATION = NUPHA,B481,109;%%
\bibitem{Binetruy:1996nx}
  P.~Binetruy, M.~K.~Gaillard and Y.~Y.~Wu,
%  ``Modular invariant formulation of multi-gaugino and matter  condensation,''
  Nucl.\ Phys.\  B {\bf 493}, 27 (1997)
  [arXiv:hep-th/9611149].
  %%CITATION = NUPHA,B493,27;%%

%--------------- BGW ------------------------------
\bibitem{Green:1984sg} %gs
  M.~B.~Green and J.~H.~Schwarz,
  %``Anomaly Cancellation In Supersymmetric D=10 Gauge Theory And Superstring
  %Theory,''
  {\em Phys.\ Lett.\ B} {\bf 149}, 117 (1984).
  %%CITATION = PHLTA,B149,117;%%
\bibitem{Derendinger:1991hq} %gs(2), dfkz
  J.~P.~Derendinger, S.~Ferrara, C.~Kounnas and F.~Zwirner,
  %``On loop corrections to string effective field theories: Field dependent
  %gauge couplings and sigma model anomalies,''
  {\em Nucl.\ Phys.\ B} {\bf 372}, 145 (1992).
  %%CITATION = NUPHA,B372,145;%%
\bibitem{LopesCardoso:1991zt} %gs1
  G.~Lopes Cardoso and B.~A.~Ovrut,
  %``A Green-Schwarz mechanism for D = 4, N=1 supergravity anomalies,''
  {\em Nucl.\ Phys.\ B} {\bf 369}, 351 (1992).
  %%CITATION = NUPHA,B369,351;%%
\bibitem{LopesCardoso:1992yd}
  G.~Lopes Cardoso and B.~A.~Ovrut,
  %``Coordinate and Kahler sigma model anomalies and their cancellation in
  %string effective field theories,''
  {\em Nucl.\ Phys.\ B} {\bf 392}, 315 (1993).
  %%CITATION = HEP-TH 9205009;%%
\bibitem{Kaplunovsky:1995jw} %kl
  V.~Kaplunovsky and J.~Louis,
  %``On Gauge couplings in string theory,''
  {\em Nucl.\ Phys.\ B} {\bf 444}, 191 (1995).
  %%CITATION = HEP-TH 9502077;%%

\bibitem{Binetruy:2000zx}
  P.~Binetruy, G.~Girardi and R.~Grimm,
  %``Supergravity couplings: A geometric formulation,''
  {\em Phys.\ Rept.}  {\bf 343}, 255 (2001).
  %%CITATION = HEP-TH 0005225;%%
\bibitem{WB}
  J.~Wess and J.~Bagger,
  {\it Supersymmetry and Supergravity},
  Princeton: Princeton University Press (1982).
\bibitem{Binetruy:1991sz} %bggm(2)
  P.~Binetruy, G.~Girardi and R.~Grimm,
  %``Linear supermultiplets and nonholomorphic gauge coupling functions,''
  {\em Phys.\ Lett.\ B} {\bf 265}, 111 (1991).
  %%CITATION = PHLTA,B265,111;%%
\bibitem{Shenker:1990uf}
  S.~H.~Shenker,
  ``The Strength Of Nonperturbative Effects In String Theory,''
  RU-90-47,
  %\href{http://www.slac.stanford.edu/spires/find/hep/www?r=ru-90-47}{SPIRES entry}
  {\it Presented at the Cargese Workshop on Random Surfaces,
  Quantum Gravity and Strings, Cargese, France, May 28 - Jun 1,
  1990}.
\bibitem{Polchinski:1994fq}
  J.~Polchinski,
  %``Combinatorics of boundaries in string theory,''
  {\em Phys.\ Rev.\  D} {\bf 50}, 6041 (1994).
  %%CITATION = PHRVA,D50,6041;%%
\bibitem{Silverstein:1996xp}
  E.~Silverstein,
  %``Duality, compactification, and e**(-1/lambda) effects in the heterotic
  %string theory,''
  {\em Phys.\ Lett.\ B} {\bf 396}, 91 (1997).
  %%CITATION = HEP-TH 9611195;%%
\bibitem{Antoniadis:1997zt}
  I.~Antoniadis, B.~Pioline and T.~R.~Taylor,
  %``Calculable e**(-1/lambda) effects,''
  {\em Nucl.\ Phys.\  B} {\bf 512}, 61 (1998).
  %%CITATION = NUPHA,B512,61;%%
\bibitem{Banks:1994sg}
  T.~Banks and M.~Dine,
  %``Coping with strongly coupled string theory,''
  {\em Phys.\ Rev.\ D} {\bf 50}, 7454 (1994).
  %%CITATION = HEP-TH 9406132;%%

\bibitem{Veneziano:1982ah}
  G.~Veneziano and S.~Yankielowicz,
  {\em Phys.\ Lett.\ B} {\bf 113}, 231 (1982).
\bibitem{Taylor:1982bp} %matter(1)
  T.~R.~Taylor, G.~Veneziano and S.~Yankielowicz,
  %``Supersymmetric QCD And Its Massless Limit: An Effective Lagrangian
  %Analysis,''
  {\em Nucl.\ Phys.\ B} {\bf 218}, 493 (1983).
  %%CITATION = NUPHA,B218,493;%%  
\bibitem{Lust:1990zi} %matter(2)
  D.~Lust and T.~R.~Taylor,
  %``Hidden Sectors With Hidden Matter,''
  {\em Phys.\ Lett.\ B} {\bf 253}, 335 (1991).
  %%CITATION = PHLTA,B253,335;%%  

\bibitem{Taylor:1985fz} %tom
  T.~R.~Taylor,
  %``Hidden Sector Of Superstring Models: An Effective Lagrangian Analysis,''
  {\em Phys.\ Lett.\ B} {\bf 164}, 43 (1985).
  %%CITATION = PHLTA,B164,43;%%
\bibitem{Binetruy:1989dk} %bmk, bg89
  P.~Binetruy and M.~K.~Gaillard,
  %``An Exact Classical Symmetry Of Effective Field Theories From Superstrings
  %And An Anomalous Source Of Observable Supersymmetry Breaking,''
  {\em Phys.\ Lett.\ B} {\bf 232}, 83 (1989).
  %%CITATION = PHLTA,B232,83;%%       
\bibitem{Gaillard:1992bt} %gt
  M.~K.~Gaillard and T.~R.~Taylor,
  %``Axion couplings and effective cutoffs in superstring compactifications,''
  {\em Nucl.\ Phys.\ B} {\bf 381}, 577 (1992).
  %%CITATION = HEP-TH 9202059;%%  
  
\bibitem{Martin:1993zk}
  S.~P.~Martin and M.~T.~Vaughn,
  %``Two Loop Renormalization Group Equations For Soft Supersymmetry Breaking
  %Couplings,''
  {\em Phys.\ Rev.\ D} {\bf 50}, 2282 (1994).
  %%CITATION = HEP-PH 9311340;%%

\bibitem{Gaillard:2003gt}
  M.~K.~Gaillard, J.~Giedt and A.~L.~Mints,
  %``Modular invariant gaugino condensation in the presence of an anomalous
  %U(1),''
  {\em Nucl.\ Phys.\ B} {\bf 700}, 205 (2004)
  [Erratum-ibid.\ {\bf B713}, 607 (2005)].
  %%CITATION = HEP-TH 0312125;%%  
\bibitem{Giedt:2001zw}
  J.~Giedt,
  %``Spectra in standard-like Z(3) orbifold models,''
  {\em Annals Phys.\ } {\bf 297}, 67 (2002).
  %%CITATION = HEP-TH 0108244;%%
\bibitem{Wu:1996en}
  Y.~Y.~Wu,
%  ``Dilaton stabilization and supersymmetry breaking by dynamical gaugino
%  condensation in the linear multiplet formalism of string effective theory,''
  [arXiv:hep-th/9610089].
  %%CITATION = HEP-TH 9610089;%%  

\bibitem{Nilles:1990jv}
  H.~P.~Nilles and M.~Olechowski,
  %``GAUGINO CONDENSATION AND DUALITY INVARIANCE,''
  {\em Phys.\ Lett.\ B} {\bf 248}, 268 (1990).
  %%CITATION = PHLTA,B248,268;%%
\bibitem{Binetruy:1990ck}
  P.~Binetruy and M.~K.~Gaillard,
  %``A Modular Invariant Formulation Of Gaugino Condensation With A Positive
  %Semidefinite Potential,''
  {\em Phys.\ Lett.\ B} {\bf 253}, 119 (1991).
  %%CITATION = PHLTA,B253,119;%%
\bibitem{Font:1990nt}
  A.~Font, L.~E.~Ibanez, D.~Lust and F.~Quevedo,
  %``SUPERSYMMETRY BREAKING FROM DUALITY INVARIANT GAUGINO CONDENSATION,''
  {\em Phys.\ Lett.\ B} {\bf 245}, 401 (1990).
  %%CITATION = PHLTA,B245,401;%%
\bibitem{Nelson:2002fk} 
  B.~D.~Nelson,
  %``Anomaly mediated supersymmetry breaking from a string theory perspective,''
  hep-ph/0211087.
  %%CITATION = HEP-PH/0211087;%%

\bibitem{Shifman:1986zi} %russians
  M.~A.~Shifman and A.~I.~Vainshtein,
  %``Solution Of The Anomaly Puzzle In Susy Gauge Theories And The Wilson
  %Operator Expansion,''
  {\em Nucl.\ Phys.\ B} {\bf 277}, 456 (1986).
\bibitem{Amati:1988ft}
  D.~Amati, K.~Konishi, Y.~Meurice, G.~C.~Rossi and G.~Veneziano,
  %``NONPERTURBATIVE ASPECTS IN SUPERSYMMETRIC GAUGE THEORIES,''
  {\em Phys.\ Rept.}  {\bf 162}, 169 (1988).
  %%CITATION = PRPLC,162,169;%%

\bibitem{Gaillard:1999et}
  M.~K.~Gaillard and B.~D.~Nelson,
%  ``Constraints on hidden sector gaugino condensation,''
  Nucl.\ Phys.\  B {\bf 571}, 3 (2000)
  [arXiv:hep-ph/9909563].
  %%CITATION = NUPHA,B571,3;%%
\bibitem{Gaillard:1999yb}
  M.~K.~Gaillard, B.~D.~Nelson and Y.~Y.~Wu,
%  ``Gaugino masses in modular invariant supergravity,''
  Phys.\ Lett.\  B {\bf 459}, 549 (1999)
  [arXiv:hep-th/9905122].
  %%CITATION = PHLTA,B459,549;%%


\bibitem{Brignole:1993dj}
  A.~Brignole, L.~E.~Ibanez and C.~Munoz,
%  ``Towards a theory of soft terms for the supersymmetric Standard Model,''
  Nucl.\ Phys.\  B {\bf 422}, 125 (1994)
  [Erratum-ibid.\  B {\bf 436}, 747 (1995)]
  [arXiv:hep-ph/9308271].
  %%CITATION = NUPHA,B422,125;%%
\bibitem{Kane:2002qp}
  G.~L.~Kane, J.~D.~Lykken, S.~Mrenna, B.~D.~Nelson, L.~T.~Wang and T.~T.~Wang,
%  ``Theory-motivated benchmark models and superpartners at the Tevatron,''
  Phys.\ Rev.\  D {\bf 67}, 045008 (2003)
  [arXiv:hep-ph/0209061].
  %%CITATION = PHRVA,D67,045008;%%



\bibitem{Binetruy:2000md}
  P.~Binetruy, M.~K.~Gaillard and B.~D.~Nelson,
%  ``One loop soft supersymmetry breaking terms in superstring effective
%  theories,''
  Nucl.\ Phys.\  B {\bf 604}, 32 (2001)
  [arXiv:hep-ph/0011081].
  %%CITATION = NUPHA,B604,32;%%    
\bibitem{Gaillard:1998bf}
  M.~K.~Gaillard,
  %``One-loop Pauli-Villars regularization of supergravity. I: Canonical gauge
  %kinetic energy,''
  {\em Phys.\ Rev.\ D} {\bf 58}, 105027 (1998).
  %%CITATION = HEP-TH 9806227;%%  
\bibitem{Gaillard:2000fk}
  M.~K.~Gaillard and B.~D.~Nelson,
  %``Quantum induced soft supersymmetry breaking in supergravity,''
  {\em Nucl.\ Phys.\ B} {\bf 588}, 197 (2000).
  %%CITATION = HEP-TH 0004170;%%   
\bibitem{Bagger:1999rd}
  J.~A.~Bagger, T.~Moroi and E.~Poppitz,
%  ``Anomaly mediation in supergravity theories,''
  JHEP {\bf 0004}, 009 (2000)
  [arXiv:hep-th/9911029].
  %%CITATION = JHEPA,0004,009;%% 
% ----- KKLT pheno paper (out of order) -----
\bibitem{Choi:2005uz}
  K.~Choi, K.~S.~Jeong and K.~i.~Okumura,
%  ``Phenomenology of mixed modulus-anomaly mediation in fluxed string
%  compactifications and brane models,''
  JHEP {\bf 0509}, 039 (2005)
  [arXiv:hep-ph/0504037].
  %%CITATION = JHEPA,0509,039;%%  

\bibitem{Allanach:2001kg} 
  B.~C.~Allanach,
  %``SOFTSUSY: a program for calculating supersymmetric spectra,''
  Comput.\ Phys.\ Commun.\  {\bf 143}, 305 (2002)
  [hep-ph/0104145].
  %%CITATION = HEP-PH/0104145;%%
\bibitem{Feng:1999zg} 
  J.~L.~Feng, K.~T.~Matchev and T.~Moroi,
  %``Focus points and naturalness in supersymmetry,''
  Phys.\ Rev.\ D {\bf 61}, 075005 (2000)
  [hep-ph/9909334].
  %%CITATION = HEP-PH/9909334;%%  
\bibitem{Chan:1997bi} 
  K.~L.~Chan, U.~Chattopadhyay and P.~Nath,
  %``Naturalness, weak scale supersymmetry and the prospect for the observation of supersymmetry at the Tevatron and at the CERN LHC,''
  Phys.\ Rev.\ D {\bf 58}, 096004 (1998)
  [hep-ph/9710473].
  %%CITATION = HEP-PH/9710473;%%  


\bibitem{Beringer:1900zz} 
  J.~Beringer {\it et al.}  [Particle Data Group Collaboration],
  %``Review of Particle Physics (RPP),''
  Phys.\ Rev.\ D {\bf 86}, 010001 (2012).
  %%CITATION = PHRVA,D86,010001;%%  
\bibitem{Bennett:2012fp} 
  C.~L.~Bennett, D.~Larson, J.~L.~Weiland, N.~Jarosik, G.~Hinshaw, N.~Odegard, K.~M.~Smith and R.~S.~Hill {\it et al.},
  %``Nine-Year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Final Maps and Results,''
  arXiv:1212.5225 [astro-ph.CO].
  %%CITATION = ARXIV:1212.5225;%%
\bibitem{Belanger:2001fz} 
  G.~Belanger, F.~Boudjema, A.~Pukhov and A.~Semenov,
  %``MicrOMEGAs: A Program for calculating the relic density in the MSSM,''
  Comput.\ Phys.\ Commun.\  {\bf 149}, 103 (2002)
  [hep-ph/0112278].
  %%CITATION = HEP-PH/0112278;%%  
\bibitem{Belanger:2004yn} 
  G.~Belanger, F.~Boudjema, A.~Pukhov and A.~Semenov,
  %``micrOMEGAs: Version 1.3,''
  Comput.\ Phys.\ Commun.\  {\bf 174}, 577 (2006)
  [hep-ph/0405253].
  %%CITATION = HEP-PH/0405253;%%  

\bibitem{Allanach:2012qd} 
  B.~C.~Allanach and M.~A.~Parker,
  %``Uncertainty in Electroweak Symmetry Breaking in the Minimal Supersymmetric Standard Model and its Impact on Searches For Supersymmetric Particles,''
  arXiv:1211.3231 [hep-ph].
  %%CITATION = ARXIV:1211.3231;%%

\bibitem{BirkedalHansen:2001is} 
  A.~Birkedal-Hansen and B.~D.~Nelson,
  %``The Role of Wino content in neutralino dark matter,''
  Phys.\ Rev.\ D {\bf 64}, 015008 (2001)
  [hep-ph/0102075].
  %%CITATION = HEP-PH/0102075;%%
\bibitem{BirkedalHansen:2002am} 
  A.~Birkedal-Hansen and B.~D.~Nelson,
  %``Relic neutralino densities and detection rates with nonuniversal gaugino masses,''
  Phys.\ Rev.\ D {\bf 67}, 095006 (2003)
  [hep-ph/0211071].
  %%CITATION = HEP-PH/0211071;%%
  %109 citations counted in INSPIRE as of 13 Mar 2013

\bibitem{Melnikov:2003xd} 
  K.~Melnikov and A.~Vainshtein,
  %``Hadronic light-by-light scattering contribution to the muon anomalous magnetic moment revisited,''
  Phys.\ Rev.\ D {\bf 70}, 113006 (2004)
  [hep-ph/0312226].
  %%CITATION = HEP-PH/0312226;%%
  %183 citations counted in INSPIRE as of 14 Feb 2013
\bibitem{Jegerlehner:2009ry} 
  F.~Jegerlehner and A.~Nyffeler,
  %``The Muon g-2,''
  Phys.\ Rept.\  {\bf 477}, 1 (2009)
  [arXiv:0902.3360 [hep-ph]].
  %%CITATION = ARXIV:0902.3360;%%
  %231 citations counted in INSPIRE as of 14 Feb 2013  

%\bibitem{Font:1989aj} 
%  A.~Font, L.~E.~Ibanez, F.~Quevedo and A.~Sierra,
%  %``The Construction of 'Realistic' Four-Dimensional Strings Through Orbifolds,''
%  Nucl.\ Phys.\ B {\bf 331}, 421 (1990).
%  %%CITATION = NUPHA,B331,421;%%
%  %238 citations counted in INSPIRE as of 14 Feb 2013  

\bibitem{Djouadi:2006bz} 
  A.~Djouadi, M.~M.~Muhlleitner and M.~Spira,
  %``Decays of supersymmetric particles: The Program SUSY-HIT (SUspect-SdecaY-Hdecay-InTerface),''
  Acta Phys.\ Polon.\ B {\bf 38}, 635 (2007)
  [hep-ph/0609292].
  %%CITATION = HEP-PH/0609292;%%
  %152 citations counted in INSPIRE as of 19 Feb 2013
\bibitem{Sjostrand:2006za} 
  T.~Sjostrand, S.~Mrenna and P.~Z.~Skands,
  %``PYTHIA 6.4 Physics and Manual,''
  JHEP {\bf 0605}, 026 (2006)
  [hep-ph/0603175].
  %%CITATION = HEP-PH/0603175;%%
  %3689 citations counted in INSPIRE as of 19 Feb 2013
\bibitem{PGS4}
  J.~Conway et al., ``PGS4: Pretty Good (Detector) Simulation'' (2009), http://physics.ucdavis.edu/~conway/research/software/pgs/pgs4-general.htm.

\bibitem{Randall:2008rw} 
  L.~Randall and D.~Tucker-Smith,
  %``Dijet Searches for Supersymmetry at the LHC,''
  Phys.\ Rev.\ Lett.\  {\bf 101}, 221803 (2008)
  [arXiv:0806.1049 [hep-ph]].
  %%CITATION = ARXIV:0806.1049;%%
  %66 citations counted in INSPIRE as of 13 Mar 2013
\bibitem{Lester:1999tx} 
  C.~G.~Lester and D.~J.~Summers,
  %``Measuring masses of semiinvisibly decaying particles pair produced at hadron colliders,''
  Phys.\ Lett.\ B {\bf 463}, 99 (1999)
  [hep-ph/9906349].
  %%CITATION = HEP-PH/9906349;%%
  %273 citations counted in INSPIRE as of 13 Mar 2013  
\bibitem{Rogan:2010kb} 
  C.~Rogan,
  %``Kinematical variables towards new dynamics at the LHC,''
  arXiv:1006.2727 [hep-ph].
  %%CITATION = ARXIV:1006.2727;%%
  %31 citations counted in INSPIRE as of 13 Mar 2013

\bibitem{Altunkaynak:2010we} 
  B.~Altunkaynak, M.~Holmes, P.~Nath, B.~D.~Nelson and G.~Peim,
  %``SUSY Discovery Potential and Benchmarks for Early Runs at $\sqrt s =7$ TeV at the LHC,''
  Phys.\ Rev.\ D {\bf 82}, 115001 (2010)
  [arXiv:1008.3423 [hep-ph]].
  %%CITATION = ARXIV:1008.3423;%%
  %25 citations counted in INSPIRE as of 11 Mar 2013

\bibitem{twiki}
https://twiki.cern.ch/twiki/bin/view/AtlasPublic/SupersymmetryPublicResults.  

%\bibitem{Tovey:2008ui} 
%  D.~R.~Tovey,
%  %``On measuring the masses of pair-produced semi-invisibly decaying particles at hadron %colliders,''
%  JHEP {\bf 0804}, 034 (2008)
%  [arXiv:0802.2879 [hep-ph]].
%  %%CITATION = ARXIV:0802.2879;%%
%  %59 citations counted in INSPIRE as of 07 Mar 2013

\bibitem{LeCompte:2011cn} 
  T.~J.~LeCompte and S.~P.~Martin,
  %``Large Hadron Collider reach for supersymmetric models with compressed mass spectra,''
  Phys.\ Rev.\ D {\bf 84}, 015004 (2011)
  [arXiv:1105.4304 [hep-ph]].
  %%CITATION = ARXIV:1105.4304;%%
  %38 citations counted in INSPIRE as of 20 Mar 2013
\bibitem{Rolbiecki:2012gn} 
  K.~Rolbiecki and K.~Sakurai,
  %``Constraining compressed supersymmetry using leptonic signatures,''
  JHEP {\bf 1210}, 071 (2012)
  [arXiv:1206.6767 [hep-ph]].
  %%CITATION = ARXIV:1206.6767;%%
  %5 citations counted in INSPIRE as of 20 Mar 2013

\bibitem{Baer:2011aa} 
  H.~Baer, V.~Barger, A.~Lessa and X.~Tata,
  %``LHC discovery potential for supersymmetry with \sqrt{s}=7 TeV and 5-30 fb^{-1},''
  Phys.\ Rev.\ D {\bf 85}, 051701 (2012)
  [arXiv:1112.3044 [hep-ph]].
  %%CITATION = ARXIV:1112.3044;%%
  %15 citations counted in INSPIRE as of 20 Mar 2013
\bibitem{Baer:2012vr} 
  H.~Baer, V.~Barger, A.~Lessa and X.~Tata,
  %``Discovery potential for SUSY at a high luminosity upgrade of LHC14,''
  Phys.\ Rev.\ D {\bf 86}, 117701 (2012)
  [arXiv:1207.4846 [hep-ph]].
  %%CITATION = ARXIV:1207.4846;%%
  %13 citations counted in INSPIRE as of 20 Mar 2013
\bibitem{Baer:2006te} 
  H.~Baer, A.~Mustafayev, E.~-K.~Park and X.~Tata,
  %``Target dark matter detection rates in models with a well-tempered neutralino,''
  JCAP {\bf 0701}, 017 (2007)
  [hep-ph/0611387].
  %%CITATION = HEP-PH/0611387;%%
  %24 citations counted in INSPIRE as of 21 Mar 2013
  
\bibitem{Aprile:2012nq} 
  E.~Aprile {\it et al.}  [XENON100 Collaboration],
  %``Dark Matter Results from 225 Live Days of XENON100 Data,''
  Phys.\ Rev.\ Lett.\  {\bf 109}, 181301 (2012)
  [arXiv:1207.5988 [astro-ph.CO]].
  %%CITATION = ARXIV:1207.5988;%%
  %166 citations counted in INSPIRE as of 18 Mar 2013

\bibitem{Akerib:2012ys} 
  D.~S.~Akerib {\it et al.}  [LUX Collaboration],
  %``The Large Underground Xenon (LUX) Experiment,''
  Nucl.\ Instrum.\ Meth.\ A {\bf 704}, 111 (2013)
  [arXiv:1211.3788 [physics.ins-det]].
  %%CITATION = ARXIV:1211.3788;%%
  %9 citations counted in INSPIRE as of 18 Mar 2013
\bibitem{Akerib:2012ak} 
  D.~S.~Akerib {\it et al.}  [LUX Collaboration],
  %``Technical Results from the Surface Run of the LUX Dark Matter Experiment,''
  arXiv:1210.4569 [astro-ph.IM].
  %%CITATION = ARXIV:1210.4569;%%
  %5 citations counted in INSPIRE as of 18 Mar 2013

\bibitem{Feldman:2010uv} 
  D.~Feldman, G.~Kane, R.~Lu and B.~D.~Nelson,
  %``Dark Matter as a Guide Toward a Light Gluino at the LHC,''
  Phys.\ Lett.\ B {\bf 687}, 363 (2010)
  [arXiv:1002.2430 [hep-ph]].
  %%CITATION = ARXIV:1002.2430;%%
  %28 citations counted in INSPIRE as of 18 Mar 2013
\bibitem{Abramowski:2013ax} 
  A.~Abramowski {\it et al.}  [H.E.S.S. Collaboration],
  %``Search for photon line-like signatures from Dark Matter annihilations with H.E.S.S,''
  Phys.\ Rev.\ Lett.\  {\bf 110}, 041301 (2013)
  [arXiv:1301.1173 [astro-ph.HE]].
  %%CITATION = ARXIV:1301.1173;%%
  %3 citations counted in INSPIRE as of 18 Mar 2013
\bibitem{Consortium:2010bc} 
  M.~Actis {\it et al.}  [CTA Consortium Collaboration],
  %``Design concepts for the Cherenkov Telescope Array CTA: An advanced facility for ground-based high-energy gamma-ray astronomy,''
  Exper.\ Astron.\  {\bf 32}, 193 (2011)
  [arXiv:1008.3703 [astro-ph.IM]].
  %%CITATION = ARXIV:1008.3703;%%
  %170 citations counted in INSPIRE as of 18 Mar 2013
\bibitem{Doro:2012xx} 
  M.~Doro {\it et al.}  [CTA Collaboration],
  %``Dark Matter and Fundamental Physics with the Cherenkov Telescope Array,''
  arXiv:1208.5356 [astro-ph.IM].
  %%CITATION = ARXIV:1208.5356;%%
  %7 citations counted in INSPIRE as of 18 Mar 2013



\bibitem{Profumo:2012tr} 
  S.~Profumo and T.~Linden,
  %``Gamma-ray Lines in the Fermi Data: is it a Bubble?,''
  JCAP {\bf 1207}, 011 (2012)
  [arXiv:1204.6047 [astro-ph.HE]].
  %%CITATION = ARXIV:1204.6047;%%
  %42 citations counted in INSPIRE as of 21 Mar 2013
\bibitem{Finkbeiner:2012ez} 
  D.~P.~Finkbeiner, M.~Su and C.~Weniger,
  %``Is the 130 GeV Line Real? A Search for Systematics in the Fermi-LAT Data,''
  JCAP {\bf 1301}, 029 (2013)
  [arXiv:1209.4562 [astro-ph.HE]].
  %%CITATION = ARXIV:1209.4562;%%
  %27 citations counted in INSPIRE as of 21 Mar 2013

  
   

 


